Aligning Language Models to Explicitly Handle Ambiguity

In interactions between users and language model agents, user utterances frequently exhibit ellipsis (omission of words or phrases) or imprecision (lack of exactness) to prioritize efficiency. This can lead to varying interpretations of the same input based on different assumptions or background knowledge. It is thus crucial for agents to adeptly handle the inherent ambiguity in queries to ensure reliability. However, even state-of-the-art large language models (LLMs) still face challenges in such scenarios, primarily due to the following hurdles: (1) LLMs are not explicitly trained to deal with ambiguous utterances; (2) the degree of ambiguity perceived by the LLMs may vary depending on the possessed knowledge. To address these issues, we propose Alignment with Perceived Ambiguity (APA), a novel pipeline that aligns LLMs to manage ambiguous queries by leveraging their own assessment of ambiguity (i.e., perceived ambiguity). Experimental results on question-answering datasets demonstrate that APA empowers LLMs to explicitly detect and manage ambiguous queries while retaining the ability to answer clear questions. Furthermore, our finding proves that APA excels beyond training with gold-standard labels, especially in out-of-distribution scenarios. The data and code are available at https://github.com/heyjoonkim/APA.

==> assets/tables/main_results_new.tex <==
\definecolor{my_gray}{HTML}{DCDCDC}
\newcolumntype{g}{>{\columncolor{my_gray}}c}

\begin{table*}[t]
    \centering    
    \resizebox{0.93\textwidth}{!}{

\begin{tabular}{lccccccccccc}
\toprule
Method & \begin{tabular}[c]{@{}c@{}}\# Train\\ Samples\end{tabular} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SituatedQA\\ (Geo)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SituatedQA\\ (Temp)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Ambig-\\ TriviaQA\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Ambig-\\ WebQuestions\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Ambig-\\ FreebaseQA\end{tabular}} \\
\cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12}
 & & F1$_{u}$ & F1$_{a}$ & F1$_{u}$ & F1$_{a}$ & F1$_{u}$ & F1$_{a}$ & F1$_{u}$ & F1$_{a}$ & F1$_{u}$ & F1$_{a}$ \\ 
 \midrule
\multicolumn{12}{l}{{\scshape Llama2 7B}} \\ 
\midrule
{\scshape Naïve} & 0 & 30.44 & 0.00 & 28.38 & 0.00 & 47.68 & 0.00 & 24.87 & 0.00 & 50.07 & 0.00 \\
{\scshape Ambiguity-aware} & 0 & 7.33 & 32.44 & 3.23 & 35.53 & 27.23 & 68.14 & 14.53 & 62.40 & 51.27 & 76.62 \\
{\scshape Sample Repetition} & 0 & 6.83 & 34.43 & 8.28 & 38.43 & 53.11 & 72.63 & 13.31 & 69.21 & 63.11 & 78.70 \\
{\scshape Self-Ask} & 0 & 29.66 & 8.18 & 26.97 & 18.48 & 48.04 & 4.99 & 20.81 & 3.02 & 48.54 & 5.03 \\
{\scshape Subset$_{\text{Random}}$} & 3,088 & 31.90 & 37.17 & 29.48 & 33.68 & 54.71 & 70.97 & 38.69 & 73.84 & 63.59 & 77.70 \\
{\scshape Subset$_{\text{Entropy}}$} & 3,088 & 39.33 & 40.84 & \underline{34.28} & 34.62 & 58.83 & 74.98 & 42.39 & 75.86 & 72.18 & 83.89 \\
{\scshape Full-set} & 10,036 & 37.67 & 41.45 & 29.59 & 36.92 & 58.1 & 71.25 & 40.46 & 73.84 & 69.97 & 80.34 \\ 
\midrule
{\scshape Ours$_{\text{Fixed}}$} & 3,088 & \underline{39.99} & \underline{41.86} & 31.74 & \underline{39.63} & \textbf{62.97} & \underline{75.50} & \textbf{49.15} & \textbf{77.07} & \textbf{73.37} & \underline{84.19} \\
{\scshape Ours$_{\text{Generated}}$} & 3,088 & \textbf{41.01} & \textbf{43.10} & \textbf{34.38} & \textbf{41.89} & \underline{59.27} & \textbf{75.74} & \underline{47.26} & \underline{76.64} & \underline{73.18} & \textbf{84.90} \\ 
\midrule
\multicolumn{12}{l}{{\scshape Mistral 7B}} \\ 
\midrule
{\scshape Naïve} & 0 & 11.29 & 0.00 & 15.34 & 0.00 & 33.19 & 0.00 & 17.85 & 0.00 & 31.37 & 0.00 \\
{\scshape Ambiguity-aware} & 0 & 3.66 & 26.01 & 8.43 & 22.48 & 26.26 & 48.43 & 8.39 & 30.52 & 32.96 & 54.91 \\
{\scshape Sample Repetition} & 0 & 7.64 & 25.31 & 7.83 & 21.13 & 29.52 & 17.04 & 8.99 & 12.10 & 27.25 & 16.31 \\
{\scshape Self-Ask} & 0 & 11.29 & 0.00 & 15.34 & 0.00 & 33.19 & 0.00 & 17.85 & 0.00 & 31.37 & 0.00 \\
{\scshape Subset$_{\text{Random}}$} & 1,382 & \underline{41.42} & 33.95 & 34.14 & 37.01 & 60.57 & 67.82 & 45.16 & 71.74 & 70.60 & 75.93 \\
{\scshape Subset$_{\text{Entropy}}$} & 1,382 & \textbf{47.34} & 29.49 & 42.00 & 32.04 & 62.17 & 67.16 & 50.93 & 71.11 & 72.94 & 77.17 \\
{\scshape Full-set} & 10,036 & 35.99 & 41.28 & 31.16 & 33.72 & 66.67 & 76.38 & 41.83 & 74.72 & 76.98 & 84.67 \\ 
\midrule
{\scshape Ours$_{\text{Fixed}}$} & 1,382 & 38.43 & \underline{41.84} & \textbf{45.01} & \textbf{43.95} & \textbf{70.70} & \textbf{83.48} & \textbf{54.02} & \textbf{81.07} & \textbf{80.84} & \textbf{90.12} \\
{\scshape Ours$_{\text{Generated}}$} & 1,382 & 39.55 & \textbf{42.07} & \underline{43.29} & \underline{40.70} & \underline{67.73} & \underline{82.14} & \underline{51.41} & \underline{79.54} & \underline{80.27} & \underline{89.22} \\ 
\midrule
\multicolumn{12}{l}{{\scshape Gemma 7B}} \\ 
\midrule
{\scshape Naïve} & 0 & 30.44 & 0.00 & 29.69 & 0.00 & 46.43 & 0.40 & 27.59 & 0.00 & 49.17 & 0.00 \\
{\scshape Ambiguity-aware} & 0 & 5.99 & 33.10 & 4.22 & 36.66 & 24.80 & 68.19 & 4.81 & 65.28 & 43.81 & 73.40 \\
{\scshape Sample Repetition} & 0 & 11.57 & 32.85 & 16.56 & 37.87 & 49.93 & 72.44 & 7.89 & 67.26 & 61.05 & 79.33 \\
{\scshape Self-Ask} & 0 & 30.44 & 0.00 & 29.69 & 0.00 & 46.43 & 0.40 & 27.59 & 0.00 & 49.17 & 0.00 \\
{\scshape Subset$_{\text{Random}}$} & 3,246 & 33.11 & 36.87 & 28.57 & 37.84 & 63.19 & 73.52 & 44.31 & 72.99 & 70.40 & 78.29 \\
{\scshape Subset$_{\text{Entropy}}$} & 3,246 & \textbf{40.19} & 38.39 & \underline{35.03} & 38.00 & 64.95 & 76.03 & 48.70 & 77.43 & 73.38 & 81.93 \\
{\scshape Full-set} & 10,036 & \underline{37.58} & 38.39 & 29.41 & 34.37 & 68.33 & 76.82 & 47.20 & 75.27 & 76.56 & 83.00 \\ 
\midrule
{\scshape Ours$_{\text{Fixed}}$} & 3,246 & 31.31 & \textbf{40.23} & \textbf{36.45} & \textbf{42.18} & \textbf{70.83} & \textbf{80.99} & \textbf{53.69} & \textbf{79.22} & \textbf{79.92} & \textbf{88.03} \\
{\scshape Ours$_{\text{Generated}}$} & 3,246 & 34.04 & \underline{39.89} & 31.72 & \underline{39.36} & \underline{69.25} & \underline{79.57} & \underline{52.96} & \underline{78.46} & \underline{79.80} & \underline{87.61} \\ 
\midrule
\multicolumn{12}{l}{{\scshape Llama2 13B}} \\ 
\midrule
{\scshape Naïve} & 0 & 34.20 & 0.00 & 30.63 & 0.00 & 40.76 & 0.00 & 21.91 & 0.00 & 43.51 & 0.00 \\
{\scshape Ambiguity-aware} & 0 & 24.08 & 21.88 & 25.16 & 23.26 & 42.80 & 45.15 & 18.60 & 31.57 & 35.00 & 39.59 \\
{\scshape Sample Repetition} & 0 & 18.74 & 33.07 & 16.87 & 36.23 & 44.69 & 66.91 & 13.84 & 61.22 & 49.21 & 68.29 \\
{\scshape Self-Ask} & 0 & 34.20 & 0.00 & 30.64 & 0.23 & 40.76 & 0.00 & 21.91 & 0.00 & 43.54 & 0.40 \\
{\scshape Subset$_{\text{Random}}$} & 3,216 & 36.26 & 36.25 & 27.52 & 35.74 & 61.61 & 73.16 & 43.13 & 73.18 & 66.22 & 77.31 \\
{\scshape Subset$_{\text{Entropy}}$} & 3,216 & \underline{37.04} & 36.96 & 27.23 & 36.78 & 60.19 & 74.01 & 41.79 & 73.92 & 64.97 & 79.29 \\
{\scshape Full-set} & 10,036 & 36.89 & \textbf{42.18} & 29.29 & 33.94 & 63.84 & 77.20 & 41.14 & 74.33 & \textbf{71.51} & 83.52 \\ 
\midrule
{\scshape Ours$_{\text{Fixed}}$} & 3,216 & \textbf{38.50} & 40.44 & \textbf{39.47} & \underline{43.59} & \underline{65.94} & \underline{77.24} & \textbf{46.76} & \textbf{77.16} & 71.27 & \underline{84.11} \\
{\scshape Ours$_{\text{Generated}}$} & 3,216 & 35.16 & \underline{40.54} & \underline{37.09} & \textbf{44.60} & \textbf{66.94} & \textbf{80.47} & \underline{44.56} & \underline{76.29} & \underline{71.47} & \textbf{85.46} \\ 
\bottomrule
\end{tabular}



    
    }
    \caption{
        Experimental results of five different OOD datasets. 
        We report unambiguous and ambiguous F1-score as F1$_{u}$ and F1$_{a}$, respectively.
        For each dataset, the \textbf{best method} is highlighted in bold and the \underline{second-best method} is underlined.
        Without the access to the ground-truth ambiguity, 
        our method outperforms all the baselines.
    }
    \label{table:main_results}
\end{table*}

==> assets/tables/main_results_wo_gemma_tmp.tex <==

\definecolor{first}{HTML}{52a6d8}
\definecolor{second}{HTML}{89ccf7}
\definecolor{third}{HTML}{caf4ff}


\begin{table*}[t]
    \centering    
    \resizebox{0.98\textwidth}{!}{

\begin{tabular}{lccccccccccc}
\toprule
Method & \begin{tabular}[c]{@{}c@{}}\# Train\\ Samples\end{tabular} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SituatedQA\\ (Geo)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SituatedQA\\ (Temp)\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Ambig-\\ TriviaQA\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Ambig-\\ WebQuestions\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Ambig-\\ FreebaseQA\end{tabular}} \\
\cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} \cmidrule(l){9-10} \cmidrule(l){11-12}
 & & F1$_{u}$ & F1$_{a}$ & F1$_{u}$ & F1$_{a}$ & F1$_{u}$ & F1$_{a}$ & F1$_{u}$ & F1$_{a}$ & F1$_{u}$ & F1$_{a}$ \\ 
 \midrule
\multicolumn{12}{l}{\textbf{{\scshape Llama2 7B}}} \\ 
\midrule
{\scshape Naïve} & 0 & 30.44 & 0.00 & 28.38 & 0.00 & 47.68 & 0.00 & 24.87 & 0.00 & 50.07 & 0.00 \\
{\scshape Ambiguity-aware} & 0 & 7.33 & 32.44 & 3.23 & 35.53 & 27.23 & 68.14 & 14.53 & 62.40 & 51.27 & 76.62 \\
{\scshape Sample Repetition} & 0 & 6.83 & 34.43 & 8.28 & \cellcolor{third}38.43 & 53.11 & 72.63 & 13.31 & 69.21 & 63.11 & 78.70 \\
{\scshape Self-Ask} & 0 & 29.66 & 8.18 & 26.97 & 18.48 & 48.04 & 4.99 & 20.81 & 3.02 & 48.54 & 5.03 \\
{\scshape Subset$_{\text{Random}}$} & 3,088 & 31.90 & 37.17 & 29.48 & 33.68 & 54.71 & 70.97 & 38.69 & 73.84 & 63.59 & 77.70 \\
{\scshape Subset$_{\text{Entropy}}$} & 3,088 & \cellcolor{third}39.33 & 40.84 & \cellcolor{second}34.28 & 34.62 & \cellcolor{third}58.83 & \cellcolor{third}74.98 & \cellcolor{third}42.39 & \cellcolor{third}75.86 & \cellcolor{third}72.18 & \cellcolor{third}83.89 \\
{\scshape Full-set} & 10,036 & 37.67 & \cellcolor{third}41.45 & 29.59 & 36.92 & 58.10 & 71.25 & 40.46 & 73.84 & 69.97 & 80.34 \\ 
\midrule
{\scshape Apa$_{\text{Fixed}}$} & 3,088 & \cellcolor{second}39.99 & \cellcolor{second}41.86 & \cellcolor{third}31.74 & \cellcolor{second}39.63 & \cellcolor{first}62.97 & \cellcolor{second}75.50 & \cellcolor{first}49.15 & \cellcolor{first}77.07 & \cellcolor{first}73.37 & \cellcolor{second}84.19 \\
{\scshape Apa$_{\text{Generated}}$} & 3,088 & \cellcolor{first}41.01 & \cellcolor{first}43.10 & \cellcolor{first}34.38 & \cellcolor{first}41.89 & \cellcolor{second}59.27 & \cellcolor{first}75.74 & \cellcolor{second}47.26 & \cellcolor{second}76.64 & \cellcolor{second}73.18 & \cellcolor{first}84.90 \\ 
\midrule
\multicolumn{12}{l}{\textbf{{\scshape Mistral 7B}}} \\ 
\midrule
{\scshape Naïve} & 0 & 11.29 & 0.00 & 15.34 & 0.00 & 33.19 & 0.00 & 17.85 & 0.00 & 31.37 & 0.00 \\
{\scshape Ambiguity-aware} & 0 & 3.66 & 26.01 & 8.43 & 22.48 & 26.26 & 48.43 & 8.39 & 30.52 & 32.96 & 54.91 \\
{\scshape Sample Repetition} & 0 & 7.64 & 25.31 & 7.83 & 21.13 & 29.52 & 17.04 & 8.99 & 12.10 & 27.25 & 16.31 \\
{\scshape Self-Ask} & 0 & 11.29 & 0.00 & 15.34 & 0.00 & 33.19 & 0.00 & 17.85 & 0.00 & 31.37 & 0.00 \\
{\scshape Subset$_{\text{Random}}$} & 1,382 & \underline{41.42} & 33.95 & 34.14 & 37.01 & 60.57 & 67.82 & 45.16 & 71.74 & 70.60 & 75.93 \\
{\scshape Subset$_{\text{Entropy}}$} & 1,382 & \textbf{47.34} & 29.49 & 42.00 & 32.04 & 62.17 & 67.16 & 50.93 & 71.11 & 72.94 & 77.17 \\
{\scshape Full-set} & 10,036 & 35.99 & 41.28 & 31.16 & 33.72 & 66.67 & 76.38 & 41.83 & 74.72 & 76.98 & 84.67 \\ 
\midrule
{\scshape Apa$_{\text{Fixed}}$} & 1,382 & 38.43 & \underline{41.84} & \textbf{45.01} & \textbf{43.95} & \textbf{70.70} & \textbf{83.48} & \textbf{54.02} & \textbf{81.07} & \textbf{80.84} & \textbf{90.12} \\
{\scshape Apa$_{\text{Generated}}$} & 1,382 & 39.55 & \textbf{42.07} & \underline{43.29} & \underline{40.70} & \underline{67.73} & \underline{82.14} & \underline{51.41} & \underline{79.54} & \underline{80.27} & \underline{89.22} \\ 
\midrule
\multicolumn{12}{l}{\textbf{{\scshape Llama2 13B}}} \\ 
\midrule
{\scshape Naïve} & 0 & 34.20 & 0.00 & 30.63 & 0.00 & 40.76 & 0.00 & 21.91 & 0.00 & 43.51 & 0.00 \\
{\scshape Ambiguity-aware} & 0 & 24.08 & 21.88 & 25.16 & 23.26 & 42.80 & 45.15 & 18.60 & 31.57 & 35.00 & 39.59 \\
{\scshape Sample Repetition} & 0 & 18.74 & 33.07 & 16.87 & 36.23 & 44.69 & 66.91 & 13.84 & 61.22 & 49.21 & 68.29 \\
{\scshape Self-Ask} & 0 & 34.20 & 0.00 & 30.64 & 0.23 & 40.76 & 0.00 & 21.91 & 0.00 & 43.54 & 0.40 \\
{\scshape Subset$_{\text{Random}}$} & 3,216 & 36.26 & 36.25 & 27.52 & 35.74 & 61.61 & 73.16 & 43.13 & 73.18 & 66.22 & 77.31 \\
{\scshape Subset$_{\text{Entropy}}$} & 3,216 & \underline{37.04} & 36.96 & 27.23 & 36.78 & 60.19 & 74.01 & 41.79 & 73.92 & 64.97 & 79.29 \\
{\scshape Full-set} & 10,036 & 36.89 & \textbf{42.18} & 29.29 & 33.94 & 63.84 & 77.20 & 41.14 & 74.33 & \textbf{71.51} & 83.52 \\ 
\midrule
{\scshape Apa$_{\text{Fixed}}$} & 3,216 & \textbf{38.50} & 40.44 & \textbf{39.47} & \underline{43.59} & \underline{65.94} & \underline{77.24} & \textbf{46.76} & \textbf{77.16} & 71.27 & \underline{84.11} \\
{\scshape Apa$_{\text{Generated}}$} & 3,216 & 35.16 & \underline{40.54} & \underline{37.09} & \textbf{44.60} & \textbf{66.94} & \textbf{80.47} & \underline{44.56} & \underline{76.29} & \underline{71.47} & \textbf{85.46} \\ 
\bottomrule
\end{tabular}



    
    }
    \caption{
        Experimental results of five different OOD datasets. 
        We report unambiguous and ambiguous F1-score as F1$_{u}$ and F1$_{a}$, respectively.
        For each dataset, the \textbf{best method} is highlighted in bold and the \underline{second-best method} is underlined.
        Without the access to the ground-truth ambiguity, 
        our method outperforms all the baselines.
    }
    \label{table:main_results}
\end{table*}

==> sections/3_methodology_old.tex <==

\section{Methodology}
% \section{Alignment with Perceived Ambiguity (APA)}
\label{sec:methodology}

\begin{figure*}[t]
    \centering
    % \includegraphics[width=\textwidth]{assets/images_tmp/pipeline6.png} 
    % \includegraphics[width=\textwidth]{assets/images/main_figure.pdf} 
    % \includegraphics[width=\textwidth]{assets/images/main_figure_wo_comments.pdf}
    % \includegraphics[width=\textwidth]{assets/images/main_figure_v2.pdf} 
    \includegraphics[width=0.98\textwidth]{assets/images/main_figure_v3.pdf} 

    \caption{
       The overall process of {\scshape APA}.
       We filter samples that a model fails to answer correctly (Stage 1)
       and let the model self-disambiguate them based on information gain between $x$ and $x_{\text{disambig}}$ (Stage 2).
       Samples with high information gain are deemed ambiguous.
       In Stage 3, the model generates a clarification request regarding the ambiguity.
       The generated clarification request is used as the label for the ambiguous query, and the model is trained accordingly (Stage 4).
       % With the ambiguous query and the disambiguation, we prompt the model to generate a clarification request regarding the ambiguity (Stage 3).
       % train the model accordingly (Stage 4).    
    }
    \label{figure:main_figure}
\end{figure*}

% The objective of our approach is to align models to explicitly handle potentially ambiguous inputs leveraging intrinsic model knowledge. 
The primary goal of our approach is to align models in a way that they can 
explicitly handle potentially ambiguous inputs leveraging the model's perceived ambiguity. 
To this end, we propose \textbf{Alignment with Perceived Ambiguity ({\scshape Apa})}, a novel four-stage alignment pipeline, illustrated in Figure \ref{figure:main_figure}.
% In this section, we first formulate the problem, and then describe each stage in detail.

\paragraph{Problem Formulation}

% In this study, we expand our input scope to not only unambiguous questions but also ambiguous ones.
% When faced with an ambiguous input $x_{\text{ambig}}$, 
In this study, we focus on open-domain question answering (QA).
For a general QA task, the goal of an LLM-based system is to generate a factually correct answer $y$,
% The goal of a QA task is to generate a factually correct answer $y$, 
given an unambiguous input $x_{\text{unambig}}$, a pre-defined inference template $t(\cdot)$, and a language model $M$.
As we expand our input scope to ambiguous queries $x_{\text{ambig}}$, 
the model is expected to generate a clarification request $y_{\text{clarify}}$
for $x_{\text{ambig}}$ to resolve the ambiguity, 
based on the belief that the user is best positioned to clarify their intent.\footnote{
    We explored alternatives for ambiguity management but found them to be impractical.
    For instance, arbitrarily selecting one of the valid answers may not accurately capture the user's intent. 
    Presenting all possible answers is often unfeasible due to the potentially vast number of valid responses.
}
% At the point of inference, 
% the model is not provided with any information regarding the ambiguity;
% only the potentially ambiguous question $x$ is provided.
% The goal is for the model to appropriately address the ambiguity inherent in $x$ and respond properly.


\subsection{Explicit Prediction Stage}
\label{pipeline:explicit}
The initial stage involves assessing 
the model's capability to correctly handle each sample
% whether the model can appropriately handle each sample
and identifying samples that the model currently fails to explicitly manage. 
We compare the model's prediction with the ground-truth label, 
where samples are categorized based on their accuracy.
% By comparing the model's prediction with the ground-truth label, samples are categorized based on their response accuracy. 
$n$ correct samples, which the model can properly handle, are collected as
$D_{\text{correct}}=\{(x^i_{\text{correct}},y^i_{\text{correct}})\}^n_{i=1}$
and incorrect samples are classified as $D_{\text{incorrect}}$.

\subsection{Perceived Ambiguity Detection Stage}

% Various factors can affect the model's incorrect response, including a lack of related model knowledge or an inability to handle ambiguity.
% As our approach focuses on ambiguity, 
The objective of this stage is to identify samples from $D_{\text{incorrect}}$ that the model perceives as ambiguous. 
Given that it is challenging for the model to explicitly express ambiguity,
we construct a proxy task to estimate the ambiguity from the model's perspective.
The task is designed to self-disambiguate $x$ and implicitly measure the perceived ambiguity. 
Specifically, the model is prompted to generate a disambiguation $\hat{x}_{\text{disambig}}$ of the input $x$.
In this process, the model leverages its intrinsic knowledge related to $x$ and generates further details.
% If $x$ lacks specifications and the model possesses related knowledge necessary to compensate,
If $x$ is underspecified and the model possesses related knowledge necessary to compensate,
then $\hat{x}_{\text{disambig}}$ would yield a higher certainty (lower entropy) for the model.
On the other hand, if $x$ requires no specification or the model lacks the necessary knowledge, 
$\hat{x}_{\text{disambig}}$ would exhibit a similar level of uncertainty to $x$.
To quantify the uncertainty associated with $x$ and $\hat{x}_{\text{disambig}}$, we employ the model's average entropy \citep{malinin2021uncertainty,ABDAR2021243}. 
Formally, the entropy of an output distribution is defined as follows:
\begin{equation}
    \mathcal{H}_{x,i} = -\sum_{v \in \mathcal{V}} p_{x,i}(v)\log p_{x,i}(v)
\end{equation}
where $p_{x,i}(v)$ is the probability of the $i^{\text{th}}$ token $v$ of a sentence $x$ from the full vocabulary set $\mathcal{V}$.
The average entropy for $x$ can be defined as:
\begin{equation}
  \mathcal{H}_{x} = \frac{1}{I} \sum_{i} \mathcal{H}_{x,i}
\end{equation}
where $x$ is composed of $I$-tokens.
We quantify the additional information gained from the disambiguation by the difference in average entropy,
% changes in input uncertainty by the difference in average entropy, 
which we define as \textbf{information gain ({\scshape Infogain})}.
The {\scshape Infogain} is defined as the following:
\begin{equation}
  \text{{\scshape Infogain}}_{x, \hat{x}_{\text{disambig}}} = \mathcal{H}_{x} - \mathcal{H}_{\hat{x}_{\text{disambig}}}
\end{equation}
% where we measure the difference of average entropy between $x$ and $x_{disambig}$.
If the disambiguation results in a meaningful specification by utilizing intrinsic knowledge, a substantial {\scshape Infogain} would be measured,
suggesting that the model considers $x$ as ambiguous.
Conversely, a negligible {\scshape Infogain} indicates that the model does not perceive $x$ as ambiguous.
Samples with {\scshape Infogain} greater than the threshold $\epsilon$ are classified as ambiguous, denoted as $x_{\text{ambig}}$.
% the initial query $x$ is ambiguous.
% Detailed analysis of the self-disambiguation is stipulated in Section \ref{sec:case_study}.
% We then measure the average entropy for both $x_{\text{disambig}}$ and $x$.
% The difference in average entropy, interpreted as the \textbf{information gain} ({\scshape Infogain}), 
% serves as an indicator of the input's ambiguity from the model's perspective. 
% A significant {\scshape Infogain} indicates that the disambiguations add clarity (reduced entropy),
% whereas a minimal {\scshape Infogain} indicates negligible additional information.
% The information gain from the disambiguation can be defined as the following:
% \begin{equation}
%   \text{{\scshape Infogain}}_{x, x_{\text{disambig}}} = \mathcal{H}_{x} - \mathcal{H}_{x_{\text{disambig}}}
% \end{equation}
% where we measure the difference of average entropy between $x$ and $x_{disambig}$.

% If the disambiguation provides additional information which makes the question more certain (less entropy), 
% the {\scshape Infogain} of $x$ would be larger.
% Conversely, if the process does not provide additional information to the model, {\scshape Infogain} would be relatively insignificant.
% Formally, the entropy of a token's probability distribution over the vocabulary is defined as:
% Formally, the entropy of an output distribution is defined as:
% \begin{equation}
%     \mathcal{H}_{x,i} = -\sum_{v \in \mathcal{V}} p_{x,i}(v)\log p_{x,i}(v)
% \end{equation}
% where $p_{x,i}(v)$ is the probability of the $i^{th}$ token $v$ of a sentence $x$ from the full vocabulary set $\mathcal{V}$.
% $\mathcal{H}_{ij}$ is the entropy of a token's probability distribution over the vocabulary at position $j$ of a sentence $i$.
% The average entropy for $x$ can be defined as:
% \begin{equation}
%   \mathcal{H}_{x} = \frac{1}{I} \sum_{i} \mathcal{H}_{x,i}
% \end{equation}

% $i=x$ and $k=x_{\text{disambig}}$.
% This is a very intuitive approach since if the model acknowledges $x$ as ambiguous, additional information would be added to the disambiguation, 
% making a more certain question.
% However, if the model assumes $x$ is unambiguous, additional information provided for the disambiguation would not affect the uncertainty of $x_{\text{disambig}}$.

% Case study of the disambiguation is stipulated in Section \ref{sec:case_study}.


\subsection{Response Construction Stage}
In this stage, we define the clarification request $y_{\text{clarify}}$ that the model should generate in response to an ambiguous query.
% when an ambiguous query is given.
We consider two approaches for response generation: Fixed response and Generated response.
% response $y_{\text{clarify}}$ to perform a clarification request when an ambiguous query is given.

\paragraph{Fixed Response}
For an ambiguous query, we randomly select a pre-defined clarification request as $y_{\text{clarify}}$.
The pre-defined clarification requests are stipulated in Appendix \ref{sec:implementation_details}.

\paragraph{Generated Response}
While a general request for clarification is feasible, 
specifying the aspect that requires clarification enhances the effectiveness of the request.
To do so, the model is provided with the query and its disambiguation to extract the factor causing the ambiguity,
thereby generating a clarification request specific to the identified factor.
Each query is thus paired with a generated clarification request $y_{\text{clarify}}$.


\subsection{Supervised Fine-Tuning (SFT) Stage}

% Model trained with the selected data is expected to properly handle $x_{\text{ambig}}$.
% To do so, we provide additional annotations for, labeling them with $y_{\text{ambig}}$.
% Specifically, samples 
% Specifically, we annotate samples
In this stage, we construct datasets for the alignment.
We label $m$ samples identified as ambiguous and constructing an ambiguous dataset $D_{\text{ambig}}=\{(x^j_{\text{ambig}},y_{\text{clarify}})\}^m_{j=1}$.
$y_{\text{clarify}}$, which was defined in the previous stage, serves as the ground-truth label for ambiguous samples.
To prevent the potential loss of the model's existing knowledge, 
we also incorporate $D_{\text{correct}}$ for training.
We balance the number of samples from both datasets so that $n=m$. 
The final training dataset is thus established as $D = D_{\text{correct}} + D_{\text{ambig}}$.
Utilizing the dataset $D=\{(x^k,y^k)\}^{n+m}_{k=1}$, the model is trained to generate ground-truth label $y$ for input $x$, 
employing the identical inference template $t(\cdot)$.
The model $M$ with parameter $\theta$ is trained as follows:
\begin{equation}
  \min_{\theta} \sum_{(x,y) \in D} \sum_{i=1}^{|y|} - \log M_{\theta}(y_i|y_{<i}, t(x))
\end{equation}
We train two versions of {\scshape Apa} based on the type of response $y_{\text{clarify}}$.
{\scshape Apa$_{\text{Fixed}}$} utilizes pre-defined responses, 
whereas {\scshape Apa$_{\text{Gen}}$} leverages generated responses as the label for ambiguous queries.
